AI Alignment: A Comprehensive Survey

AI alignment aims to make AI systems behave in line with human intentions and values. As AI systems grow more capable, so do risks from misalignment. To provide a comprehensive and up-to-date overview of the alignment field, in this survey, we delve into the core concepts, methodology, and practice of alignment. First, we identify four principles as the key objectives of AI alignment: Robustness, Interpretability, Controllability, and Ethicality (RICE). Guided by these four principles, we outline the landscape of current alignment research and decompose them into two key components: forward alignment and backward alignment. The former aims to make AI systems aligned via alignment training, while the latter aims to gain evidence about the systems' alignment and govern them appropriately to avoid exacerbating misalignment risks. On forward alignment, we discuss techniques for learning from feedback and learning under distribution shift. On backward alignment, we discuss assurance techniques and governance practices. We also release and continually update the website (www.alignmentsurvey.com) which features tutorials, collections of papers, blog posts, and other resources.

==> files/intro.tex <==

\section{Introduction (Under Reconstruction)}
\label{sec:introduction}

\subsection{The Motivation of Alignment}

\subsubsection{Risks}

Recent advancements have seen the increasing application of capable AI systems in complex domains (\S\ref{sec:agi}), such as applications of autonomous agents based on Large Language Models (LLMs) \citep{xi2023rise, wang2023survey} and the utilization of Deep Reinforcement Learning (DRL) for the control of nuclear fusion \citep{degrave2022magnetic}. The increasing capabilities and deployment in high-stakes domains come with heightened risks. Various undesirable behaviors exhibited by advanced AI systems (\textit{e.g.}, manipulation \citep{turner2019optimal, perez2022discovering, carroll_characterizing_2023, steinhardt_emergent_2023, sharma2023towards} and deception \citep{park2023ai}) have raised concerns about the hazards from AI systems. 

Consequently, these concerns have catalyzed research efforts in \emph{AI alignment} \citep{bostrom2013existential, ord2020precipice, christian2020alignment, bucknall2022current}. AI alignment aims to make AI systems behave in line with human intentions and values \citep{leike2018scalable} -- it focuses on the intent and objective of AI systems, as opposed to their capabilities. Failures of alignment (\emph{i.e.}, misalignment) are among the most salient causes of potential harm from AI. Mechanisms underlying these failures include \emph{reward hacking} \citep{pan2022effects} and \emph{goal misgeneralization} \citep{shah2022goal}, which are further amplified by \emph{double edge components} such as situational awareness \citep{berglund2023taken}, broadly-scoped goals \citep{ngo2022alignment}, mesa-optimization objectives \citep{hubinger2019risks}, and access to increased resources \citep{shevlane2023model} (\S\ref{sec:challenges-of-alignment}).

Alignment efforts to address these failures focus on accomplishing four key objectives (\S\ref{sec:RICE}): Robustness, Interpretability, Controllability, and Ethicality (\textbf{RICE}). Current research and practice on alignment consist of four areas (\S\ref{sec:scope}): Learning from Feedback (\S\ref{sec:learning-from-feedback}), Learning under Distributional Shift (\S\ref{sec:distribution}), Assurance (\S\ref{sec:assurance}), and Governance (\S\ref{sec:governance}). The four objectives and the four areas are not in one-to-one correspondence. Each individual area often serves more than one alignment objective, and vice versa (see Table \ref{tab:category-over-RICE}).

In this survey, we introduce the concept, methodology, and practice of AI alignment and discuss its potential future directions.\footnote{To help beginners interested in this field learn more effectively, we highlight resources about alignment techniques. More details can be found at \url{www.alignmentsurvey.com/resources}}

% \subsection{The Alignment Problem}
\label{sec:motivation-of-alignment}

The motivation for alignment is a three-step argument, each step building upon the previous one: (1) Deep learning-based systems (or applications) have an increasingly large impact on society and bring significant risks (\S\ref{sec:agi}); (2) Misalignment represents a significant source of risks (\S\ref{sec:agi}); and (3) Alignment research and practice address risks stemming from misaligned systems (\textit{e.g.}, power-seeking behaviors) (\S\ref{sec:RICE}).

% \subsubsection{The Prospect and Impact of AGI}\label{sec:agi}

In the past decade, deep learning has made significant strides, leading to the emergence of large-scale neural networks with remarkable capabilities in various domains. 
These advances represent a transition from symbolic systems \citep{smolensky1987connectionist, goel2022looking} to deep learning-based systems \citep{mnih2015human,openai2023gpt4}. Such systems have led to progress in many settings, including game environments \citep{silver2017mastering,berner2019dota,kaufmann2023champion} and more intricate, even high-stakes, real-world scenarios \citep{ruff2021alphafold,degrave2022magnetic}. In particular, LLMs have exhibited improved capabilities in multi-step reasoning \citep{wei2022chain, wang2022self} and cross-task generalization \citep{brown2020language, askell2021general}. These abilities are strengthened with increased training time, training data, and parameter size \citep{kaplan2020scaling, srivastava2022beyond, hoffmann2022training}.


With improved capabilities come increased risks. Some undesirable behaviors of LLMs (\textit{e.g.}, untruthful answers \citep{bang2023multitask}, sycophancy \citep{perez2022discovering, sharma2023towards}, and deception \citep{jacob2023, park2023ai}) worsen with increased model scale \citep{perez2022discovering}, resulting in concerns about advanced AI systems that are hard to control. Moreover, emerging trends such as \emph{LLM-based agents} \citep{xi2023rise,wang2023survey} also raise concerns about the system's controllability and ethicality \citep{chan2023harms}. Looking further ahead, the development of increasingly competent AI systems opens up the possibility of realizing Artificial General Intelligence (AGI) in the foreseeable future, \textit{i.e.}, systems can match or surpass human intelligence in all relevant aspects \citep{bubeck2023sparks}. This could bring extensive opportunities \citep{manyika2017future} such as automation \citep{west2018future}, efficiency improvements \citep{furman2019ai}, and rapid technological progress \citep{korinek2021technological}, but also come with serious risks \citep{statement_on_ai_risk_2023,critch2023tasra}, such as safety concerns \citep{hendrycks2022x}, biases and inequalities \citep{ntoutsi2020bias}, and large-scale risks from superhuman capabilities~\citep{nick2014superintelligence,rogueai}. Taking biases as an example, cutting-edge LLMs manifest discernible biases about gender, sexual identity, and immigrant status among others \citep{perez2022discovering}, which could reinforce existing inequalities.



Within the large-scale risks from superhuman capabilities \citep{nick2014superintelligence}, it has been conjectured that global catastrophic risks (\textit{i.e.}, risks of severe harms on a global scale) \citep{bostrom2011global,hendrycks2023overview, gov_uk_2023} and existential risks (\textit{i.e.}, risks that threaten the destruction of humanity's long-term potential) \citep{ord2020precipice} from advanced AI systems are especially worrying. These concerns are elaborated in first-principle deductive arguments \citep{firstprinc,rogueai}, evolutionary analysis \citep{hendrycks2023natural}, and concrete scenario mapping \citep{christiano2019failure,threatmodel2022}. In \citet{statement_on_ai_risk_2023}, leading AI scientists and other notable figures stated that \textit{Mitigating the risk of extinction from AI should be a global priority alongside other societal-scale risks such as pandemics and nuclear war}. The median researcher surveyed by \citet{stein2022expert} at NeurIPS 2021 and ICML 2021 reported a 5\% chance that the long-run effect of advanced AI on humanity would be \textit{extremely bad (\textit{e.g.}, human extinction)}, and 36\% of NLP researchers surveyed by \citet{michael2022nlp} self-reported to believe that \textit{AI could produce catastrophic outcomes in this century, on the level of all-out nuclear war}. \footnote{However, survey results may hinge upon the exact wording of the questions and should be taken with caution.} Existential risks from AI also include risks of lock-in, stagnation, and more \citep{bostrom2013existential,hendrycks2022x}, in addition to extinction risks.\footnote{\textit{Existential} and \textit{extinction} risks are two concepts that are often mixed up. The latter is a subset of the former.} The latest news is that the UK will host the world's first global AI Safety Summit, gathering international governments, leading AI companies, civil society groups, and research experts. Its objectives are to:
(1) assess the risks associated with AI, particularly at the cutting edge of its development; (2) explore how these risks can be mitigated through internationally coordinated efforts\footnote{Source from \url{https://www.gov.uk/government/topical-events/ai-safety-summit-2023}.}.



Specifically, current cutting-edge AI systems have exhibited multiple classes of undesirable or harmful behaviors that may contrast with human intentions (\textit{e.g.}, powerful-seeking and manipulation) \citep{si2022so,pan2023machiavelli}, and similar worries about more advanced systems have also been raised \citep{critch2020ai, statement_on_ai_risk_2023}.\footnote{See \S\ref{sec:challenges-of-alignment} for an introduction to specific misalignment challenges.} These undesirable or harmful behaviors not compliant with human intentions, known as \textit{misalignment} of AI systems\footnote{Some of the misaligned behaviors are less risky (\textit{e.g.}, the agent fails to clean the room as you want), however, some of them are dangerous for systems applied in the high-stakes environment (\textit{e.g.}, the control of nuclear fusion \citep{degrave2022magnetic})}, can naturally occur even without misuse by malicious actors and represent a significant source of risks from AI, including safety hazards \citep{hendrycks2021unsolved} and potential existential risks \citep{hendrycks2023overview}.\footnote{It should be noted that misalignment cannot cover all sources of risks brought by Deep learning-based systems and other factors such as misuse and negligence also contribute to risks on society. See \S\ref{sec:ai-safety-beyond} for discussing AI safety beyond alignment.} These large-scale risks are significant in size due to the non-trivial likelihoods of (1) building superintelligent AI systems, (2) those AI systems pursuing large-scale goals, (3) those goals are misaligned with human intentions and values, and (4) this misalignment leads to humans losing control of humanity's future trajectory \citep{firstprinc}.

Solving the risks brought by misalignment requires \textit{alignment techniques} of AI systems to ensure the objectives of the AI system are in accordance with human intentions and values, thereby averting unintended and unfavorable outcomes. More importantly, we expect the alignment techniques to be scaled to harder tasks and significantly advanced AI systems that are even smarter than humans. A potential solution is \textit{Super Alignment}\footnote{For more details on Super Alignment, you can refer to \url{https://openai.com/blog/introducing-superalignment}.}, which aims to build a roughly human-level automated alignment researcher, thereby using vast amounts of compute to scale up and iteratively align superintelligence \citep{superalignment}.




% \subsubsection{The Objectives of Alignment: RICE}
\label{sec:RICE}




\begin{tcolorbox}[colback=gray!20, colframe=gray!50, sharp corners, center title]
\centering
\textit{\large How can we build AI systems that behave in line with human intentions and values?}
\end{tcolorbox}

There is not a universally accepted definition of \textit{alignment}. Before embarking on this discussion, we must clarify what we mean by alignment goals. \citet{leike2018scalable} frame it as the agent alignment problem, posing the question: ``How can we create agents that behave in accordance with the user intentions?'' One could also focus on super-human AI systems \citep{superalignment} and ask: ``How do we ensure AI systems much smarter than humans follow human intent?'' A consistent theme in these discussions is the focus on \textit{human intentions}. To clearly define alignment goals, it's imperative to accurately characterize human intentions, a challenging task, as noted by \citet{kenton2021alignment}. For instance, the term \textit{human} can represent various entities ranging from an individual to humanity. \citet{gabriel2020artificial} breaks down intentions into several categories, such as instruction (follow my direct orders), expressed intentions (act on my underlying wishes), revealed preferences (reflect my behavior-based preferences), and so on.

Concretely, we characterize the objectives of alignment with four principles: Robustness, Interpretability, Controllability, and Ethicality (\textbf{RICE}). Figure \ref{fig:RICE} summarizes the principles, and Table \ref{tab:category-over-RICE} gives the correspondence between alignment research directions covered in the survey and the principles to which they contribute. The following is a detailed explanation of the four principles.

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{assets/rice.pdf}
    \caption{The \textbf{RICE} principles define four key characteristics that an aligned system should possess, in no particular order: (1) \textbf{Robustness} states that the system's stability needs to be guaranteed across various environments; (2) \textbf{Interpretability} states that the operation and decision-making process of the system should be clear and understandable; (3) \textbf{Controllability} states that the system should be under the guidance and control of humans; (4) \textbf{Ethicality} states that the system should adhere to society's norms and values. These four principles guide the alignment of an AI system with human intentions and values. They are not end goals in themselves but intermediate objectives in service of alignment.}
    \label{fig:RICE}
\end{figure}

\begin{itemize}
\item \textbf{Robustness}
Robustness refers to the resilience of AI systems when operating across diverse scenarios \citep{dietterich2017steps} or under adversarial pressures \citep{Runder2021b}, especially the correctness of its objective in addition to capabilities. Robust AI systems should be able to cope with black swan events \citep{taleb2007black} and long-tailed risks \citep{hendrycks2021unsolved}, as well as a diverse array of adversarial pressures \citep{song2018constructing,chakraborty2021survey}. For example, an aligned language model ought to refuse requests to behave harmfully, but models can be made to cause harm through jailbreak prompts and other adversarial attacks \citep{carlini2023aligned, zou2023universal, shah2023scalable}. Instead, an adversarially robust model should behave as intended even when facing inputs designed to cause failure. As AI systems find increasing deployment in high-stakes domains such as the military and economy \citep{Jacob2020}, there will be a growing need to ensure their resilience against unexpected disruptions and adversarial attacks, given that even momentary failures can yield catastrophic consequences \citep{kirilenko2017flash, oecd2021, Runder2021b}. Aligned systems should consistently maintain robustness throughout their lifecycle \citep{russell2019human}.

\item \textbf{Interpretability}
Interpretability demands that we can understand the AI systems' inner reasoning, especially the inner workings of opaque neural networks \citep{rauker2023toward}. Straightforward approaches to alignment assessments, such as behavioral evaluations, potentially suffer from dishonest behaviors \citep{turpin2023language,park2023ai,jacob2023} or deceptive alignment \citep{hubinger2019deceptive,carranza2023deceptive} of AI systems. One way to cope with this issue is to make AI systems honest, non-concealing, and non-manipulative \citep{pacchiardi2023catch,radhakrishnan2023question,carroll2023characterizing}. Alternatively, we could build interpretability tools that peek into the inner concepts and mechanisms within neural networks \citep{elhage2021mathematical,meng2022locating}. In addition to enabling safety assessments, interpretability also makes decision-making processes accessible and comprehensible to users and stakeholders, thus enabling human supervision. As AI systems assume a more pivotal role in real-world decision-making processes and high-stakes settings \citep{holzinger2017we}, it becomes imperative to demystify the decision-making process rather than allowing it to remain an opaque black box \citep{Deepmind2018, Runder2021a}. 

\item \textbf{Controllability}
Controllability is a necessary attribute that ensures the actions and decision-making processes of a system remain subject to human oversight and intervention. It guarantees that human intervention can promptly rectify any deviations or errors in the system's behavior \citep{soares2015corrigibility,hadfield2016off}. As AI technology advances, an increasing body of research is expressing growing concerns about the controllability of these potent systems \citep{critch2020ai, unite2023, arcevalscollab}. When an AI system begins to pursue goals that contradict its human designers, it can manifest capabilities that pose significant risks, including deception, manipulation, and power-seeking behaviors \citep{shevlane2023model, arcevalscollab}.
The objective of controllability is sharply focused on enabling scalable human oversight during the training process \citep{bowman2022measuring}, as well as \emph{corrigibility} of AI systems (\emph{i.e.}, not resisting shutdown or objective modification during deployment) \citep{soares2015corrigibility}.

\item \textbf{Ethicality}
Ethicality refers to a system's unwavering commitment to uphold human norms and values within its decision-making and actions. Here, the norms and values include both moral guidelines and other social norms/values. It ensures that the system avoids actions that violate ethical norms or social conventions, such as exhibiting bias against specific groups \citep{buolamwini2018gender,zhang2018mitigating,noble2018algorithms,kearns2019ethical,raji2020saving,berk2021fairness}, causing harm to individuals \citep{hendrycks2021aligning,hendrycks2021would,pan2023machiavelli}, and lacking diversity or equality when aggregating preferences \citep{CIPwhitepaper}. A significant body of research is dedicated to developing ethical frameworks for AI systems \citep{hagendorff2020ethics,pankowska2020framework}. This emphasis on imbuing AI systems with ethical principles is necessary for their integration into society \citep{winfield2019machine}.
\end{itemize}


% \paragraph{Comparing the RICE Principles with Their Alternatives} The \textbf{RICE} principles represent a succinct summary of alignment objectives from the perspective of alignment and coexistence of humans and machines. Several previous works have put forth guidelines concerning AI systems. Asimov's Laws can be regarded as the earliest exploration of human-machine coexistence, emphasizing that robots should benefit humans and the difficulty of achieving this \citep{Asimov1942}. On another front, the FATE principle (Fairness, Accountability, Transparency, and Ethics) \citep{memarian2023fairness} leans towards defining high-level qualities AI systems should possess within the human-machine coexistence ecosystem. We aspire to answer the human-machine coexistence question from the standpoint of human governors and designers, considering what steps are necessary to ensure the builder AI systems are aligned with human intentions and values. Furthermore, some standards emphasize narrowly defined safety, such as the 3H standard (Helpful, Honest, and Harmless) \citep{askell2021general} and governmental agency proposals \citep{white2023}. We aim to expand upon these standards by introducing other crucial dimensions, including Controllability and Robustness. 



\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}
\begin{table}[t]
\caption{Relationships between alignment research directions covered in the survey and the \textbf{RICE} principles, featuring the individual objectives each research direction aims to achieve. Filled circles stand for primary objectives, and unfilled circles stand for secondary objectives.}
\label{tab:category-over-RICE}
\centering
\resizebox{\textwidth}{!}{
% \usepackage{color}
% \usepackage{tabularray}
\begin{tblr}{
  columns = {c, m, c, m, m, m, m},
  row{1} = {c},
  row{2} = {c},
  row{3} = {c},
  row{4} = {c},
  row{5} = {c},
  row{6} = {c},
  row{7} = {c},
  row{8} = {c},
  row{9} = {c},
  row{10} = {c},
  row{11} = {c},
  row{12} = {c},
  row{13} = {c},
  row{14} = {c},
  row{15} = {c},
  row{16} = {c},
  row{17} = {c},
  row{18} = {c},
  row{19} = {c},
  row{22} = {c},
  row{23} = {c},
  row{24} = {c},
  row{25} = {c},
  row{26} = {c},
  cell{1}{1} = {c=3}{},
  cell{1}{4} = {c=4}{},
  cell{3}{1} = {r=8}{},
  cell{3}{2} = {c=2}{},
  cell{4}{2} = {r=2}{},
  cell{6}{2} = {r=5}{},
  cell{11}{1} = {r=5}{},
  cell{11}{2} = {r=3}{},
  cell{14}{2} = {r=2}{},
  cell{16}{1} = {r=6}{},
  cell{16}{2} = {r=3}{},
  cell{19}{2} = {c=2}{},
  cell{20}{2} = {r=2}{c},
  cell{20}{3} = {c},
  cell{20}{4} = {c},
  cell{20}{6} = {c},
  cell{20}{7} = {c},
  cell{21}{3} = {c},
  cell{21}{4} = {c},
  cell{21}{7} = {c},
  cell{22}{1} = {r=5}{},
  cell{22}{2} = {r=3}{},
  cell{25}{2} = {c=2}{},
  cell{26}{2} = {c=2}{},
  hline{1,3,27} = {-}{0.08em},
  hline{2,11,16,22} = {-}{},
  hline{4,6,14,19-20,25-26} = {2-7}{},
  hline{5,7-10,12-13,15,17-18,21,23-24} = {3-7}{},
}
\textbf{Alignment Research Directions \& Practices} &  &  & \textbf{Objectives} & & & \\

\textbf{Category}  & \textbf{Direction}  & \textbf{Method} & \textbf{Robustness} & \textbf{Interpretability} & \textbf{Controllability} & \textbf{Ethicality} \\

{Learning from \\ Feedback\\ (\S\ref{sec:learning-from-feedback})} & 
Preference Modeling (\S\ref{ssec:preference_modeling})& {\Large$\circ$} & & {\Large$\bullet$}& {\Large$\circ$}     \\

 & {Policy Learning\\ (\S\ref{ssec:policy_learning})} & {RL/PbRL/IRL/\\ Imitation Learning} &  &  & {\Large$\circ$}   &  \\
 
 & & RLHF & {\Large$\circ$} &  & {\Large$\bullet$} &{\Large$\bullet$} \\
 
 & {Scalable Oversight\\ (\S\ref{ssec:scalable_oversight})} & RL$x$F  & {\Large$\circ$} &  & {\Large$\bullet$} & {\Large$\bullet$}   \\
  
 & & IDA & & {\Large$\circ$} & {\Large$\bullet$} & \\
 
 & & RRM & & & {\Large$\bullet$} &  \\
 
 & & Debate & & {\Large$\circ$} & {\Large$\bullet$} & \\
 
 & & CIRL & {\Large$\circ$} & {\Large$\circ$} & {\Large$\bullet$}& {\Large$\circ$}     \\
 
{Learning under\\ Distribution Shift\\ (\S\ref{sec:distribution})}  & {Algorithmic\\ Interventions\\ (\S\ref{sec:alg-inter})} & DRO & {\Large$\bullet$} & & & \\

 &  & IRM/REx  & {\Large$\bullet$} & & & \\
 
 & & CBFT  & {\Large$\bullet$}  & & & \\
 
 & {Data Distribution\\ Interventions (\S\ref{sec:data-inter})}     & Adversarial Training & {\Large$\bullet$} & & {\Large$\circ$} & \\
 
 & & Cooperative Training & {\Large$\bullet$} & & & {\Large$\bullet$} \\
 
Assurance (\S\ref{sec:assurance}) & {Safety\\ Evaluations\\ (\S\ref{sec:safe})} & {Social Concern\\ Evaluations} & {\Large$\circ$} & {\Large$\circ$} & & {\Large$\bullet$}   \\

 & & {Extreme Risk\\ Evaluations} & & {\Large$\circ$} & {\Large$\bullet$} & {\Large$\circ$} \\
 
 & & Red Teaming & {\Large$\bullet$} & & {\Large$\circ$} & {\Large$\bullet$}   \\
 
 & Interpretability (\S\ref{sec:interpretability}) & & & {\Large$\bullet$} & {\Large$\circ$} & \\
 
 & {Human Values\\ Verification (\S\ref{sec:human-values-alignment})} & 
 {Learning/Evaluating\\ Moral Values} & & & {\Large$\circ$} & {\Large$\bullet$}   \\
 
 & & {Game Theory for\\ Cooperative AI} & {\Large$\circ$} & & & {\Large$\bullet$}   \\
 
Governance (\S\ref{sec:governance}) & {Multi-Stakeholder\\ Approach (\S\ref{sec:multi-stake})} & Government & {\Large$\bullet$}   & {\Large$\bullet$} & {\Large$\bullet$}  & {\Large$\bullet$} \\

 & & Industry & {\Large$\bullet$} & {\Large$\bullet$} & {\Large$\bullet$} & {\Large$\bullet$} \\
 
 & & Third Parties & {\Large$\bullet$} & {\Large$\bullet$} & {\Large$\bullet$} & {\Large$\bullet$} \\
 
 & International Governance (\S\ref{sec:intl-gov}) & & {\Large$\bullet$} & {\Large$\bullet$} & {\Large$\bullet$} & {\Large$\bullet$}   \\
 
 & Open-Source Governance (\S\ref{sec:o-s-g}) & & {\Large$\bullet$} & {\Large$\bullet$} &{\Large$\bullet$} & {\Large$\bullet$}   
 
\end{tblr}
}
\end{table}

\subsubsection{Causes}
\label{sec:challenges-of-alignment}
In the above sections, we discuss the alignment problems and the scope of alignment, pointing out that misaligned AI systems may take unintended actions that give rise to undesirable consequences. To offer a deeper understanding of alignment, we aim to analyze why and how the misaligned issue occurs, paving the way for the following sections about alignment techniques. 
Guided by our \textit{alignment cycle} (see Figure \ref{fig:maindiagram}), we try to elucidate the failure modes of alignment and analyze misaligned behaviors, thereby suggesting directions for future research. 
In \S\ref{sec:mechanism}, we give an overview of common failure modes, and in \S\ref{sec:feedback-induced}, we focus on the mechanism of feedback-induced misalignment. In \S\ref{sec:hazardous}, our emphasis shifts towards a more focused examination of misaligned behaviors and dangerous capabilities. Furthermore, we introduce the concept of \textit{double edge components}, which offer benefits for enhancing the capabilities of future advanced systems but also bear the potential for hazardous outcomes.

% \subsubsection{Overview of Failure Modes}
\label{sec:mechanism}
In order to illustrate the misalignment issue, we give an overview of alignment failure modes in this section, most of which can be categorized into \textit{reward hacking}\footnote{\textit{Reward hacking} can also be broadly considered as a kind of \textit{specification gaming}.} and \textit{goal misgeneralization}.

The learning process of RL can be deconstructed into two distinct phases: firstly, the creation of an agent primed for reward optimization, and secondly, the establishment of a reward process that furnishes the agent with appropriate reward signals. Within the framework of the Markov Reward Process \citep{marbach2001simulation, puterman2014markov, sutton2018reinforcement}, the former phase can be seen as the learning process related to the transition model (\textit{e.g.}, model-based RL agents \citep{moerland2023model}), or the development of specialized algorithms. The latter phase can be viewed as the construction of proxy rewards, which aim to approximate the true rewards derived from sources (\textit{e.g.}, human preferences or environment) \citep{ng2000algorithms,leike2018scalable}.


% \paragraph{Reward Hacking}
% In practice, proxy rewards are often easy to optimize and measure, yet they frequently fall short of capturing the full spectrum of the actual rewards \citep{pan2022effects}. This limitation is denoted as \textit{misspecified rewards} \footnote{A similar definition is reward misidentification in which scenario the reward function is only partially identifiable. For more details on reward misidentification, see \textit{e.g.}, \citet{tien2022causal,skalse2023invariance}}. The pursuit of optimization based on such misspecified rewards may lead to a phenomenon known as \textit{reward hacking}, wherein agents may appear highly proficient according to specific metrics but fall short when evaluated against human standards \citep{amodei2016concrete,everitt2017reinforcement}. For instance, in \textit{CoastRunners} game, the agent consistently prioritizes collecting gain-enhancing items over maximizing speed  \citep{clark2016faulty}.
The discrepancy between proxy rewards and true rewards often manifests as a sharp phase transition in the reward curve  \citep{ibarz2018reward}.
Furthermore, \citet{skalse2022defining} defines the hackability of rewards and provides insights into the fundamental mechanism of this phase transition, highlighting that the inappropriate simplification of the reward function can be a key factor contributing to reward hacking.


Misspecified rewards often occur due to a neglect of severe criteria for the outcomes, thus making specification too broad and potentially easily hacked \citep{specification2020victoria}. More than poor reward design \citep{ng1999policy}, the choice of training environment and simulator with bugs \citep{bullet2022} can both lead to AI systems failing to satisfy intended objectives. These problems stem from task specification, broadly defined as \textit{specification gaming}, which refers to AI systems exploiting loopholes in the task specification without achieving intended outcomes.\footnote{For more instances about specification gaming, please see \citet{instances2020}} \citep{specification2020victoria}

\textit{Reward tampering} can be considered a special case of reward hacking \citep{everitt2021reward, skalse2022defining}, referring to AI systems corrupting the reward signals generation process \citep{ring2011delusion, everitt2018alignment, kumar2020realab}. \citet{everitt2021reward} delves into the subproblems encountered by RL agents: (1) \textit{tampering of reward function}, where the agent inappropriately interferes with the reward function itself, and (2) \textit{tampering of reward function input}, which entails corruption within the process responsible for translating environmental states into inputs for the reward function.
When the reward function is formulated through feedback from human supervisors, models can directly influence the provision of feedback (\textit{e.g.}, AI systems intentionally generate challenging responses for humans to comprehend and judge, leading to feedback collapse) \citep{leike2018scalable}. Since task specification has its physical instantiation (\textit{e.g.}, memory registers storing the reward signals), the AI systems deployed in the real world have the potential to practice manipulation behaviors, resulting in more hazardous outcomes \citep{specification2020victoria}.

% \paragraph{Goal Misgeneralization} \emph{Goal misgeneralization} is another failure mode, wherein the agent actively pursues objectives distinct from the training objectives in deployment while retaining the capabilities it acquired during training \citep{koch2021objective, di2022goal}.\footnote{More discussion about Goal Misgeneralization can be found in \S\ref{sec:chal-dis}.} For instance, in \textit{CoinRun} games,  the agent frequently prefers reaching the end of a level, often neglecting relocated coins during testing scenarios \citep{koch2021objective}.
\citet{di2022goal} draw attention to the fundamental disparity between capability generalization and goal generalization, emphasizing how the inductive biases inherent in the model and its training algorithm may inadvertently prime the model to learn a proxy objective that diverges from the intended initial objective when faced with the testing distribution. It implies that even with perfect reward specification, goal misgeneralization can occur when faced with distribution shifts \citep{amodei2016concrete, shah2022goal}. It should be noted that goal misgeneralization can occur in any learning system, not limited to RL since the core feature is the pursuit of unintended goals \citep{examples2022}.
Moreover, it might be more dangerous if advanced AI systems escape control and leverage their capabilities to bring about undesirable states \citep{nick2014superintelligence, zhuang2020consequences}.


% \subsubsection{Feedback-Induced Misalignment}
\label{sec:feedback-induced}
With the proliferation of advanced AI systems, the challenges related to reward hacking and goal misgeneralization have become increasingly pronounced in open-ended scenarios \citep{paulus2017deep, knox2023reward}. \citet{gao2023scaling} underscores that more capable agents tend to exploit misspecified rewards to a greater extent. While many current AI systems are primarily driven by self-supervision, it's worth noting that a substantial portion relies on feedback rewards derived from human advisors \citep{bai2022training}, allowing us to introduce the mechanism of feedback-induced misalignment. The misalignment issues are particularly pressing in open-ended scenarios, and we can attribute them to two primary factors:
\begin{itemize}[left=0.3cm]
\item \textbf{Limitations of Human Feedback}.
 During the training of LLMs, inconsistencies can arise from human data annotators (\textit{e.g.}, the varied cultural backgrounds of these annotators can introduce implicit biases \citep{peng2022investigations}) \citep{openai2023gpt4}. Moreover, they might even introduce biases deliberately, leading to untruthful preference data \citep{casper2023open}.  For complex tasks that are hard for humans to evaluate (\textit{e.g.}, the value of game state), these challenges \footnote{As AI systems are deployed into more complex tasks, these difficulties amplify, necessitating novel solutions such as \textit{scalable oversight} \citep{cotra2018iterated}.} become even more salient \citep{irving2018ai}.

\item \textbf{Limitations of Reward Modeling}.
Training reward models using comparison feedback can pose significant challenges in accurately capturing human values. For example, these models may unconsciously learn suboptimal or incomplete objectives, resulting in reward hacking \citep{zhuang2020consequences,skalse2022defining}.
Meanwhile, using a single reward model may struggle to capture and specify the values of a diverse human society \citep{casper2023open}.

\end{itemize}


Additionally, \citet{huang2022inner,andreas2022language,kim2023language} demonstrate that advanced AI systems exhibit patterns of goal pursuit and multi-step reasoning capability, which further aggravate the situation if the reward is not well-defined  \citep{ngo2022alignment,yang2023foundation}. 


% \paragraph{Discussion} It can be challenging to distinguish goal misgeneralization from reward hacking in specific cases. For instance \citep{examples2022}, LLMs are trained to generate \textit{harmless, honest, and helpful} outputs, but LLMs may occasionally produce harmful outputs in detail, which seemingly receive low rewards in testing distribution (which could be seen as goal misgeneralization). 
However, in cases where labelers are incentivized to assign high rewards to responses deemed more helpful during the labeling process, the scenarios above \footnote{Harmful but detailed responses} actually receive high rewards and represent a form of specification gaming (or reward hacking). The distinction between these two scenarios can be vague at times.



More research is needed to analyze the failure modes, gain a deeper understanding of reward hacking, and develop effective methods for detecting and mitigating goal misgeneralization to address the challenges of misaligned advanced AI systems.

% \subsubsection{Misaligned Behaviors and Outcomes}
\label{sec:hazardous}
\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{assets/failures.pdf}
\caption{Dangerous Capabilities. Advanced AI systems would be incentivized to seek power because power will help them achieve their given objectives. Powerful AI systems might hack computer systems, manipulate humans, control and develop weaponry, and perform ethical violations while avoiding a shutdown. Original copyright belongs to wiki \citep{wiki}, based on which we have made further adjustments. We will further discuss these issues in \S\ref{sec:hazardous}.}

\label{fig:failure}
\end{figure}

Drawing from the misalignment mechanism, optimizing for a non-robust proxy may result in misaligned behaviors, potentially leading to even more catastrophic outcomes. This section delves into a detailed exposition of specific \textbf{misaligned behaviors} ($\bullet$) and introduces what we term \textbf{double edge components} (+). These components are designed to enhance the capability of AI systems in handling real-world settings but also potentially exacerbate misalignment issues. {It should be noted that some of these \textbf{double edge components} (+) remain speculative. Nevertheless, it is imperative to discuss their potential impact before it is too late, as the transition from controlled to uncontrolled advanced AI systems may be just one step away \citep{ngo2020continuing}.} With increased model scale, a class of \textbf{dangerous capabilities} (*) \citep{shevlane2023model} could also emerge. The \textbf {dangerous capabilities} (*) are concrete tasks the AI system could carry out; they may not necessarily be misaligned in themselves but are instrumental to actualizing extreme risks.

We first introduce the \textbf{double edge components} (+) and analyze how they act on AI systems. 
\begin{itemize}[left=0.35cm]
    \item [+] \textbf{Situational Awareness}. AI systems may gain the ability to effectively acquire and use knowledge about its status, its position in the broader environment, its avenues for influencing this environment, and the potential reactions of the world (including humans) to its actions~\citep{cotra2022,berglund2023taken}. Similar behaviors have been observed in LLMs \citep{jonas2022,evan2023}. Knowing the situation can help the model better understand human intent, finish tasks within its ability, and search for outlier help if needed. However, such knowledge also paves the way for advanced methods of reward hacking, heightened deception/manipulation skills, and an increased propensity to chase instrumental subgoals \citep{ngo2022alignment}.  Consequently, it should be given priority when evaluating potentially hazardous capabilities in AI models, alongside eight other key competencies \citep{shevlane2023model}. A highly relevant discussion is whether language models possess \textit{world models} \citep{lecun2022path,li2022emergent}.
    \item [+] \textbf{Broadly-Scoped Goals}. Advanced AI systems are expected to develop objectives that span long timeframes, deal with complex tasks, and operate in open-ended settings \citep{ngo2022alignment}. Engaging in broadly-scoped planning can empower AI systems to generalize better on the OOD settings and serve as valuable assistants in realms such as human healthcare. However, it can also bring about the risk of encouraging manipulating behaviors (\textit{e.g.}, AI systems may take some \textit{bad} actions to achieve human happiness, such as persuading them to do high-pressure jobs \citep{jacob2023} \footnote{This behavior is due to models' over-optimization for broadly-scoped goals and this over-optimization is hard to perceive by humans}). Intuitively, one approach to mitigate this risk is to confine the optimizable objectives to short-sighted ones, such as predicting only the next word, thereby preventing over-ambitious planning, but such approaches limit systems' utility and may fail; for instance, source text data (\textit{e.g.}, fiction) can help AI systems understand the intent and belief of the roles, and thus longer-term goal-directed behavior can be elicited  \citep{andreas2022language}. Additionally, techniques such as RL-based fine-tuning \citep{christiano2017deep,ouyang2022training} or the application of chain-of-thought prompts \citep{wei2022chain} can enable models to adapt their acquired knowledge about planning to pave the way for broadly-scoped planning objectives \citep{jacob2023}.
    \item [+] \textbf{Mesa-Optimization Objectives}. The learned policy may pursue inside objectives \emph{when the learned policy itself functions as an optimizer} (\textit{i.e.}, \textit{mesa-optimizer}). However, this optimizer's objectives may not align with the objectives specified by the training signals, and optimization for these misaligned goals may lead to systems out of control \citep{hubinger2019risks}. \citet{freeman2019learning,wijmans2023emergence} indicate that AI systems may possess implicit goal-directed planning and manifest emergent capabilities during the generalization phase.
    \item [+] \textbf{Access to Increased Resources}. Future AI systems may gain access to websites and engage in real-world actions, potentially yielding a more substantial impact on the world \citep{nakano2021webgpt}. They may disseminate false information, deceive users, disrupt network security, and, in more dire scenarios, be compromised by malicious actors for ill purposes. Moreover, their increased access to data and resources can facilitate \textit{self-proliferation}, posing existential risks \citep{shevlane2023model}.
\end{itemize}

Furthermore, we illustrate the \textbf{misaligned behaviors} ($\bullet$) and \textbf{dangerous capabilities} (*) to show specific misalignment issues and provide directions for future alignment evaluation research.
\begin{itemize}[left=0.3cm]
    \item \textbf{Power-Seeking Behaviors}. AI systems may exhibit behaviors that attempt to gain control over resources and humans and then exert that control to achieve its assigned goal \citep{carlsmith2022power}. The intuitive reason why such behaviors may occur is the observation that for almost any optimization objective (\textit{e.g.}, investment returns), the optimal policy to maximize that quantity would involve power-seeking behaviors (\textit{e.g.}, manipulating the market), assuming the absence of solid safety and morality constraints. \citet{omohundro2008basic,bostrom2012superintelligent,nick2014superintelligence} have argued that power-seeking is an \textit{instrumental subgoal} which is instrumentally helpful for a wide range of objectives and may, therefore, be favored by AI systems. \citet{turner2019optimal} also proved that in MDPs that satisfy some standard assumptions, the optimal policies tend to be power-seeking. \citet{perez2022discovering} prompt LLMs to test their tendency to suggest power-seeking behaviors, find significant levels of such tendencies, and show that RLHF strengthens them. This also holds for other instrumental subgoals such as self-preservation \citep{bostrom2012superintelligent,shevlane2023model}. Another notable line of research is \emph{side-effect avoidance}, which aims to address power-seeking behaviors by penalizing agentic systems for having too much influence over the environment. It covers RL systems \citep{eysenbach2017leave,turner2020avoiding,krakovna2020avoiding} and symbolic planning systems \citep{klassen2022planning}.
    
    \item \textbf{Measurement Tampering}. Multiple model measurements can be manipulated by models, resulting in an illusion of favorable outcomes, even in cases where the desired objectives are not met. This deceptive practice can be seen as a specific kind of specification gaming, enabling models to escape detection techniques and presenting a false impression of alignment. \citet{roger2023measurement} create datasets to assess detection techniques related to measurement tampering and establish the current state of the art in this field. It is noteworthy that such manipulation of measurements has the potential to amplify deceptive behavior, resulting in unforeseen and unpredictable outcomes.

    \item \textbf{Untruthful Output}. AI systems such as LLMs can produce either unintentionally or deliberately inaccurate output. Such untruthful output may diverge from established resources or lack verifiability, commonly referred to as \textit{hallucination} \citep{bang2023multitask, zhao2023survey}. More concerning is the phenomenon wherein LLMs may selectively provide erroneous responses to users who exhibit lower levels of education\footnote{Such behaviors bare termed \textit{sandbagging} \citep{perez2022discovering}. They may have been learned from web text during pre-training, which suggests that supervised learning can also bring about deceptive behaviors if those behaviors are present in training data.} \citep{perez2022discovering}. The behavior (also known as sycophancy) appears emergently at scale \citep{cotra2021,perez2022discovering} and untruthful output has the potential to engender deception, especially as advanced AI systems gain greater access to online resources and websites \citep{jacob2023}.

    \item \textbf{Deceptive Alignment \& Manipulation}.  Manipulation \& Deceptive Alignment is a class of behaviors that exploit the incompetence of human evaluators or users \citep{hubinger2019deceptive,carroll2023characterizing,carranza2023deceptive} and even manipulate the training process through \textit{gradient hacking} \citep{ngogra2022} or \textit{reward tampering} \citep{kumar2020realab}. These behaviors can potentially make detecting and addressing misaligned behaviors much harder. 

    \textit{Deceptive Alignment}: Misaligned AI systems may deliberately mislead their human supervisors instead of adhering to the intended task. Such deceptive behavior has already manifested in AI systems that employ evolutionary algorithms \citep{wilke2001evolution,lehman2020surprising,hendrycks2021unsolved}. In these cases, agents evolved the capacity to differentiate between their evaluation and training environments. They adopted a strategic pessimistic response approach during the evaluation process, intentionally reducing their reproduction rate within a scheduling program \citep{lehman2020surprising}. Furthermore, AI systems may engage in intentional behaviors that superficially align with the reward signal, aiming to maximize rewards from human supervisors \citep{ouyang2022training}. It is noteworthy that current large language models occasionally generate inaccurate or suboptimal responses despite having the capacity to provide more accurate answers \cite {lin2021truthfulqa,chen2021evaluating}. These instances of deceptive behavior present significant challenges. They undermine the ability of human advisors to offer reliable feedback (as humans cannot make sure whether the outputs of the AI models are truthful and faithful). Moreover, such deceptive behaviors can propagate false beliefs and misinformation, contaminating online information sources \citep{hendrycks2021unsolved}.


    \textit{Manipulation}: Advanced AI systems can effectively influence individuals' beliefs, even when these beliefs are not aligned with the truth \citep{shevlane2023model}. These systems can produce deceptive or inaccurate output or even deceive human advisors to attain deceptive alignment. Such systems can even persuade individuals to take actions that may lead to hazardous outcomes \citep{openai2023gpt4}.
    
    
    Early-stage indications of such behaviors are present in LLMs,\footnote{Namely, the \emph{untruthful output} that we discuss above.} recommender systems (where the system influences the users' preferences) \citep{kalimeris2021preference, krueger2020hidden, evans2021user, adomavicius2022recommender}, and RL agents (where agents trained from human feedback adopt policies to trick human evaluators) \citep{learning2017dario}. Also, current LLMs already possess the capability needed for deception. In \citet{sciadvadh}, it has been found that GPT-3 is super-human capable of producing convincing disinformation. Given all these early-stage indications, it is plausible that more advanced AI systems may exhibit more serious deceptive/manipulative behaviors.

    \item \textbf{Collectively Harmful Behaviors}. AI systems have the potential to take actions that are seemingly benign in isolation but become problematic in multi-agent or societal contexts. Classical game theory offers simplistic models for understanding these behaviors. For instance, \citet{phelps2023investigating} evaluates GPT-3.5's performance in the iterated prisoner's dilemma and other social dilemmas, revealing limitations in the model's cooperative capabilities. \citet{perolat2017multiagent} executes a parallel analysis focused on common-pool resource allocation. To mitigate such challenges, the emergent field of Cooperative AI \citep{dafoe2020open,dafoe2021cooperative} has been advancing as an active research frontier. However, beyond studies grounded in simplified game-theoretical frameworks, there is a pressing need for research in more realistic, socially complex settings \citep{singh2014norms}. In these environments, agents are numerous and diverse, encompassing AI systems and human actors \citep{critch2020ai}. Furthermore, the complexity of these settings is amplified by the presence of unique tools for modulating AI behavior, such as social institutions and norms \citep{singh2014norms}. \footnote{We cover cooperative AI research in \S\ref{sec:cooperative-ai-training} and \S\ref{subsec:formal-ethics-coop}.}

    \item \textbf{Violation of Ethics}. Unethical behaviors in AI systems pertain to actions that counteract the common good or breach moral standards—such as those causing harm to others. These adverse behaviors often stem from omitting essential human values during the AI system's design or introducing unsuitable or obsolete values into the system \citep{boddington2020ai,kenward2021machine}. Research efforts addressing these shortcomings span the domain of \textit{machine ethics} \citep{yu2018building, winfield2019machine, tolmeijer2020implementations} and delve into pivotal questions, \textit{e.g.}, \textit{whom should AI align with?} \citep{korinek2022aligned, santurkar2023whose}, among other concerns.
     \item [*] \textbf{Dangerous Capabilities}. Figure \ref{fig:failure} outlines the dangerous capabilities that advanced AI systems might have. As AI systems are deployed in the real world, they may pose risks to society in many ways (\textit{e.g.}, hack computer systems, escape containment, and even violate ethics). They may hide unwanted behaviors, fool human supervisors, and seek more resources to become more powerful. Moreover, \textbf{double edge components} (+) may intensify the danger and lead to more hazardous outcomes, even resulting in existential risks \citep{bostrom2013existential}.
\end{itemize}

\subsection{The Scope of Alignment}\label{sec:scope}

\subsubsection{The Objectives of Alignment: RICE}

\begin{figure}[t]  
    \centering
    \includegraphics[width=1.0\linewidth]{assets/architecture.pdf}
    \caption{The Alignment Cycle. (1) \textbf{\color{myred}Forward Alignment} (alignment training) produces \textit{trained systems} based on \textit{alignment requirements}; (2) \textbf{\color{myblue}Backward Alignment} (alignment refinement) ensures the practical alignment of \textit{trained systems} and revises \textit{alignment requirements}; (3) The cycle is repeated until reaching a sufficient level of alignment. Notably, although Backward Alignment has the end goal of ensuring the practical alignment of \textit{trained systems}, it is carried out all throughout the system's lifecycle in service of this goal, including before, during, after training, and also after deployment \citep{shevlane2023model,koessler2023risk,schuett2023towards}.}
    \label{fig:maindiagram}
\end{figure}

In this section, we focus on illustrating the scope of AI alignment: we constructed the alignment process as an \textit{alignment cycle} and decomposed it into \textit{Forward Alignment Process} and \textit{Backward Alignment Process}\footnote{From this point and throughout the survey, for convenience, we refer to ``Forward Alignment'' and ``Backward Alignment''.} (\S\ref{sec:forward-backward}). Specifically, we discuss the role of \textit{human values} in alignment (\S\ref{sec:values-in-intro}) and further analyze AI safety problems beyond alignment (\S\ref{sec:ai-safety-beyond}).

\subsubsection{The Forward and Backward Process}
\label{sec:forward-backward}
We decompose alignment into {\color{myred}\textbf{Forward Alignment}} (alignment training) (\S\ref{sec:learning-from-feedback}, \S\ref{sec:distribution}) and {\color{myblue}\textbf{Backward Alignment}} (alignment refinement) (\S\ref{sec:assurance}, \S\ref{sec:governance}). 
Forward Alignment aims to produce trained systems that follow alignment requirements.\footnote{Here, \emph{alignment requirements} refer to an operationalized specification of the alignment properties that are desired of the AI systems, including, for example, which concrete forms of robustness/interpretability/controllability/ethicality we require, in what specific settings we require them, and how they could be measured.}
We decompose this task into Learning from Feedback (\S\ref{sec:learning-from-feedback}) and Learning under Distribution Shift 
 (\S\ref{sec:distribution}). 
Backward Alignment aims to ensure the practical alignment of the trained systems by performing evaluations in both simplistic and realistic environments and setting up regulatory guardrails to handle real-world complexities,\textit{i.e.}, Assurance 
(\S\ref{sec:assurance}). It also covers the creation and enforcement of rules that ensure the safe development and deployment of AI systems, \textit{i.e.}, Governance (\S\ref{sec:governance}). At the same time, backward alignment updates the alignment requirements based on the evaluation and monitoring of the systems, both pre-deployment and post-deployment. These updated requirements then inform the next round of alignment training. 

The two phases, forward and backward alignment, thus form a cycle where each phase produces or updates the input of the next phase (see Figure \ref{fig:maindiagram}). This cycle, what we call \textit{the alignment cycle}, is repeated to produce increasingly aligned AI systems. We see alignment as a dynamic process in which all standards and practices should be continually assessed and updated. Notably, Backward Alignment (including the Assurance of alignment in AI systems and the Governance of AI systems) efforts occur throughout the entire alignment cycle, as opposed to only after training. As argued in \citet{shevlane2023model,koessler2023risk}, alignment and risk evaluations should occur in every stage of the system's lifecycle, including before, during, after training, and post-deployment. Similarly, regulatory measures for every phase of the system's lifecycle have been proposed and discussed \citep{schuett2023towards, anderljung2023frontier}.

The survey is structured around four core pillars: Learning from Feedback (\S\ref{sec:learning-from-feedback}) and Learning under Distribution Shift (\S\ref{sec:distribution}), which constitute the components of Forward Alignment; and Assurance (\S\ref{sec:assurance}) and Governance (\S\ref{sec:governance}) which form the elements of Backward Alignment. The subsequent paragraphs provide a concise introduction to each pillar, clarifying how they synergistically contribute to a comprehensive framework for AI alignment.

\begin{itemize}[left=0.3cm]
\item\textbf{{Learning from Feedback} {\normalfont(\S\ref{sec:learning-from-feedback})}} \textit{Learning from feedback} concerns the question of \textit{during alignment training, how do we provide and use feedback to behaviors of the trained AI system?} It takes an input-behavior pair as given and only concerns how to provide and use feedback on this pair.\footnote{Here, \textit{behavior} is broadly defined also to include the system's internal reasoning, which can be examined via interpretability tools (see \S\ref{sec:interpretability}).} In the context of LLMs, a typical solution is reinforcement learning from human feedback (RLHF) \citep{christiano2017deep, bai2022training}, where human evaluators provide feedback by comparing alternative answers from the chat model, and the feedback is used via Reinforcement Learning (RL) against a trained reward model. Despite its popularity, RLHF faces many challenges \citep{pandey2022modeling, casper2023open, tien2022causal}, overcoming which has been a primary objective of alignment research \citep{bowman2022measuring}, and is one primary focus of the section. An outstanding challenge here is \textit{scalable oversight} (\S\ref{ssec:scalable_oversight}), \textit{i.e.}, providing high-quality feedback on super-human capable AI systems that operate in complex situations beyond the grasp of human evaluators, where the behaviors of AI systems may not be easily comprehended and evaluated by humans \citep{bowman2022measuring}. Another challenge is the problem of providing feedback on ethicality, which is approached by the direction of machine ethics \citep{anderson2011machine, tolmeijer2020implementations}. On the ethics front, misalignment could also stem from neglecting critical dimensions of variance in values, such as underrepresenting certain demographic groups in feedback data \citep{santurkar2023whose}. There have also been work combining feedback mechanisms with \emph{social choice} methods to produce a more rational and equitable aggregation of preferences \citep{CIPwhitepaper} (see \S\ref{sec:values-in-intro}).


\item\textbf{{Learning under Distribution Shift} {\normalfont(\S\ref{sec:distribution})}} In contrast to learning from feedback, which holds input fixed, this pillar focuses specifically on the cases where the distribution of input changes, \textit{i.e.}, where distribution shift occurs \citep{krueger2020hidden,thulasidasan2021effective,hendrycks2021many}. More specifically, it focuses on the preservation of \emph{alignment properties} (\emph{i.e.}, adherence to human intentions and values) under distribution shift, as opposed to that of model capabilities.
In other words, it asks how we can ensure an AI system well-aligned on the training distribution will also be well-aligned when deployed in the real world. One challenge related to distribution shift is \textit{goal misgeneralization}, where, under the training distribution, the intended objective for the AI system (\textit{e.g.}, following human's real intentions) is indistinguishable from other unaligned objectives (\textit{e.g.}, gaining human approval regardless of means). The system learns the latter, which leads to unaligned behaviors in deployment distribution \citep{di2022goal,shah2022goal}. 
Another related challenge is \textit{auto-induced distribution shift} (ADS), where an AI system changes its input distribution to maximize reward \citep{krueger2020hidden,perdomo2020performative}. An example would be a recommender system shaping user preferences \citep{kalimeris2021preference,adomavicius2022recommender}. Both goal misgeneralization and ADS are closely linked to deceptive behaviors \citep{park2023ai} and manipulative behaviors \citep{carroll2023characterizing} in AI systems, potentially serving as their causes. Interventions that address distribution shift include \emph{algorithmic interventions} (\S\ref{sec:alg-inter}), which changes the training process to improve reliability under other distributions, and \emph{data distribution interventions} (\S\ref{sec:data-inter}) which expands the training distribution to reduce the discrepancy between training and deployment distributions. The former includes methods like Risk Extrapolation (REx) \citep{krueger2021out} and Connectivity-based Fine-tuning (CBFT) \citep{lubana2023mechanistic}. The latter includes adversarial training (\S\ref{sec:adversarial-training}) \citep{song2018constructing,bai2021recent} which augments training input distribution with adversarial inputs, and cooperative training (\S\ref{sec:cooperative-ai-training}) \citep{dafoe2020open, dafoe2021cooperative} which aims to address the distribution gap between single-agent and multi-agent settings.\footnote{Cooperative Training aims to make AI systems more cooperative in multi-agent settings. This cooperativeness addresses multi-agent failure modes where the AI system's behavior appears benign and rational in isolation but becomes problematic within social or multi-agent scenarios~\citep{critch2020ai}; see \emph{collectively harmful behaviors} in \S\ref{sec:hazardous} for a more detailed account.} 

\item\textbf{{Assurance} {\normalfont(\S\ref{sec:assurance})}} Once an AI system has undergone forward alignment, we still need to gain confidence about its alignment before deploying it \citep{ukassurance, anderljung2023frontier}. Such is the role of \textit{assurance}: assessing the alignment of trained AI systems. Methodologies of assurance include safety evaluations \citep{perez2022discovering,shevlane2023model} (\S\ref{sec:safe}) and more advanced methods such as interpretability techniques \citep{olah_building_2018} (\S\ref{sec:interpretability}) and red teaming \citep{perez2022red} (\S\ref{subsec:red teaming}). The scope of assurance also encompasses the verification of system's alignment with human values, including formal theories focused on provable cooperativeness \citep{dafoe2020open, dafoe2021cooperative} and ethicality \citep{anderson2011machine, tolmeijer2020implementations}, and also a wide range of empirical and experimental methods (\S\ref{sec:human-values-alignment}). Assurance takes place throughout the lifecycle of AI systems, including before, during, after training, and post-deployment, as opposed to only after training \citep{shevlane2023model,koessler2023risk}.\footnote{Furthermore, it's noteworthy that many techniques here are also applicable in the training process, \textit{e.g.}, red teaming is a key component of adversarial training (see \S\ref{sec:adversarial-training}), and interpretability can help with giving feedback \citep{burns_discovering_2022}.}


\item\textbf{{Governance} {\normalfont(\S\ref{sec:governance})}} Assurance alone cannot provide full confidence about a system's practical alignment since it does not account for real-world complexities. This necessitates governance efforts of AI systems that focus on their alignment and safety and cover the entire lifecycle of the systems (\S\ref{sec:the-role-of-ai-governance}). We discuss the multi-stakeholder approach of AI governance, including the governmental regulations \citep{anderljung2023frontier}, the lab self-governance \citep{schuett2023towards}, and the third-party practice, such as auditing \citep{shevlane2023model,koessler2023risk} (\S\ref{sec:multi-stake}). We also highlight several open problems in AI governance, including the pressing challenge of open-source governance (the governance of open-source models and the question of whether to open-source highly capable models) \citep{seger2023open}, and the importance of international coordination in AI governance \citep{ho2023international} (\S\ref{sec:open-problems}). In addition to policy research, we also cover key actions from both the public and the private sector.
\end{itemize}

\paragraph{Comparison with Inner/Outer Decomposition} Our \emph{alignment cycle} framework (see Figure \ref{fig:maindiagram}) decomposes alignment into four pillars: Learning from Feedback, Learning under Distribution Shift, Assurance and Governance organized into a circular process. The design principle for this framework is three-fold: Practical (making sure pillars directly correspond to specific practices in specific stages in the system's lifecycle), Concrete (pointing to specific research directions as opposed to general themes), and Up-To-Date (accommodating and emphasizing latest developments in the alignment field). Recently, the decomposition of alignment into \emph{outer alignment} and \emph{inner alignment} has become popular in the alignment literature \citep{inneralignment}. Outer alignment refers to the wishes of designers in accordance with the actual task specification (\textit{e.g.}, goal \& reward) used to build AI systems. And inner alignment is the consistency between task specification and the specification that the AI systems behaviors reflect \citep{vkrpara}. However, many criticisms have also been made about this characterization, including that it is ambiguous and is understood by different people to mean different things \citep{innerouter} and that it creates unnecessary difficulties by carving out problems that are not necessary conditions for success \citep{harderprob}. Some have tried to remove the ambiguity by pinning down the specific causes of inner/outer misalignment and proposed, for example, \emph{goal misspecification} and \emph{goal misgeneralization} \citep{shah2022goal,vkrpara}. Learning from Feedback (approximately corresponding to \emph{goal misspecification} and \emph{outer alignment}) and Learning under Distribution shift (approximately corresponding to \emph{goal misgeneralization} and \emph{inner alignment}) in our framework tries to further improve upon the inner/outer decomposition by clarifying the exact approaches taken to address the challenges and resolving the ambiguity. Assurance and Governance, on the other hand, expands the scope to cover topics beyond outer and inner alignment.

\paragraph{Theoretical Research in Alignment} The alignment research literature also contains a wealth of theoretical work \citep{amodei2016concrete,everitt2018agi,hendrycks2021unsolved}. These works often propose new directions and provide a foundation for practical and empirical research to build upon. We give a brief overview of this body of theoretical research below:

\begin{itemize}[left=0.3cm]

\item {\textbf{Conceptual Frameworks}}. Some theoretical work proposes conceptual frameworks or characterizes subproblems within alignment. Examples include \emph{instrumental convergence} (wherein highly intelligent agents tend to pursue a common set of sub-goals, such as self-preservation and power-seeking) \citep{omohundro2008basic,bostrom2012superintelligent}, \emph{mesa-optimization} (wherein the learned ML model performs optimization within itself during inference) \citep{hubinger2019risks}, and specific proposals for building aligned systems, such as \emph{approval-directed agents} (wherein the AI system does not pursue goals, but seek the human's idealized post hoc approval of action consequences) \citep{oesterheld2021approval,christiano2022approval}. \citet{hadfield2019incomplete,cotra2021the} have drawn inspiration from economics, linking problems in alignment with markets and principal-agent problems in economics. \citet{elk_intro,elk_summary} have proposed the problem of \emph{eliciting latent knowledge} of advanced AI systems and have explored high-level approaches to the problem.

\item {\textbf{Mathematical Formulations}}. Other theoretical works have aimed to formulate sub-problems within alignment mathematically and seek formal solutions. \citet{soares2015corrigibility} formulates the problem of corrigibility (\textit{i.e.}, ensuring AI systems are incentivized to allow shutdown or objective modification by the instructor). \citet{benson2016formalizing} gives a mathematical formulation of instrumental convergence. \citet{hadfield2016off} proposes the \textit{off-switch game} to model the uncontrollability of AI agents. \citet{turner2019optimal} proves the power-seeking tendencies of optimal policies in Markov decision processes (MDPs) under certain assumptions. 
\citet{everitt2016avoiding} proposes \emph{value reinforcement learning} to eliminate incentives for reward hacking \citep{skalse2022defining, pan2022effects}. Another avenue of research, designated as \emph{agent foundations}~\citep{soares2017agent}, aims to establish a rigorous formal framework for the agency that deals appropriately with unresolved issues of embedded agency \citep{demski2019embedded}. This body of work explores a variety of key topics, including decision theory~\citep{soares2015toward}, corrigibility~\citep{soares2015corrigibility}, value learning~\citep{soares2018value}, logical uncertainty \citep{garrabrant2016logical}, and open-source game theory \citep{critch2022cooperative} among others.

\end{itemize}

\subsubsection{Human Values in Alignment}\label{sec:values-in-intro}

The inclusion of \emph{Ethicality} in our RICE principles signifies the critical role of human values in alignment. AI systems should be aligned not only with value-neutral human preferences (such as intentions for AI systems to carry out tasks) but also with moral and ethical considerations. These efforts are referred to as \emph{value alignment} \citep{gabriel2020artificial,gabriel2021challenge}.\footnote{Although this term has also been used in other ways, such as to refer to alignment in general \citep{yuan2022situ}.} Considerations of human values are embedded in all parts of alignment -- indeed, alignment research topics dedicated to human values are present in all four sections of our survey. Therefore, to provide a more holistic picture of these research topics, here we give an overview of them before delving into their details in each individual section. 

We classify alignment research on human values into three main themes: (1) \emph{Ethical and social values} which aims to teach AI systems right from wrong, (2) \emph{cooperative AI} which aims to specifically foster cooperative behaviors from AI systems, and (3) \emph{Addressing social complexities} which provides apparatus for the modeling of multi-agent and social dynamics.

\paragraph{Ethical and Social Values} Human values inherently possess a strong degree of abstraction and uncertainty. \citet{macintyre2013after} even points out that modern society lacks a unified value standard, and the value differences between people of different cultures can be vast. This raises the significant challenge of determining which human values we should align with. Although universally consistent human values may not exist, there are still some values that are reflected across different cultures. In the sections below, we discuss these from the perspectives of \textbf{Machine Ethics}, \textbf{Fairness}, and \textbf{Cross-Cultural Values in Social Psychology}.

\begin{itemize}[left=0.3cm]
\item \textbf{Machine Ethics}. In contrast to much of alignment research which aligns AI systems with human preferences in general (encompassing both value-laden ones and value-neutral ones), \emph{machine ethics} have specifically focused on instilling appropriate moral values into AI systems \citep{yu2018building, winfield2019machine, tolmeijer2020implementations}. This line of work started early on in the context of symbolic and statistical AI systems \citep{anderson2005towards,arkoudas2005toward,anderson2007status}, and later expanded to include large-scale datasets \citep{hendrycks2021aligning,pan2023machiavelli} and deep learning-based/LLM-based methods \citep{jiang2021can,jin2022make}. 
We cover the formal branch of machine ethics in \S\ref{subsec:formal-ethics-coop}.

\item \textbf{Fairness}. Although there are controversies ~\citep{verma2018fairness, saxena2019fairness}, the definition of fairness is relatively clear compared to other human values. Specifically, it is the absence of any prejudice or favoritism toward an individual or group based on their inherent or acquired characteristics ~\citep{mehrabi2021survey}. Therefore, there has been extensive research on AI fairness. These methods range from reducing data biases before training ~\citep{d2017conscientious, bellamy2018ai}, to minimizing unfairness introduced during the training process ~\citep{berk2017convex}, and finally addressing instances of unfairness that were not successfully learned during training ~\citep{xu2018fairgan}.

\item \textbf{Cross-Cultural Values in Social Psychology}. In the field of social psychology, numerous studies have focused on exploring clusters of values that exist among cross-cultural human communities, leading to the development of various cross-cultural values scales. The Allport-Vernon-Lindzey value system ~\citep{allport1955becoming} posited that understanding an individual's philosophical values constitutes a critical foundation for assessing their belief system. They devised a value scale comprising six primary value types, each representing people's preferences and concerns regarding various aspects of life. \citet{messick1968motivational, mcclintock1982social, liebrand1984effect, van1997development} introduced and improved a quantifiable method, namely social value orientation (SVO), to assess an individual's social value inclination. It utilizes quantitative approaches to evaluate how individuals allocate benefits to themselves and others, reflecting their social value orientation, such as altruism, individualism, \textit{etc.} In subsequent work, \citet{murphy2011measuring, murphy2014social} introduced the Slider Measure, which can be used to precisely assess the SVO value as a continuous angle based on the subject's option to some specific questions. \citet{rokeach1973nature} developed a values inventory comprising 36 values, consisting of 18 terminal values representing desired end-states and 18 instrumental values signifying means to achieve those end-states. 
\citet{schwartz1992universals, schwartz1994there} conducted comprehensive questionnaire surveys in 20 diverse countries known as the Schwartz Value Survey. This study identified ten values that are universally recognized, regardless of culture, language, or location.
These studies have all laid a solid theoretical foundation for establishing what kind of values AI should be aligned with. However, they are constrained by the historical context of their research and may not maintain strong universality across different times and cultures.

\end{itemize}

\paragraph{Cooperative AI} Arguably, the most exciting aspect of multi-agent interaction is cooperation, and cooperation failure is the most worrying aspect of multi-agent interaction. As an example of AI cooperation failure, the \emph{2010 Flash Crash} led to a temporary loss of trillions of market value in 2 minutes and was caused in part by interactions between high-frequency algorithmic traders \citep{kirilenko2017flash}. Therefore, there is a need to implement mechanisms ensuring cooperation in agent-like AI systems and the environments they're operating within \citep{dafoe2021cooperative}. The high-level design principles and low-level implementations of such mechanisms fall into the domain of \emph{Cooperative AI} \citep{dafoe2020open}. In addition, Cooperative AI also studies human cooperation through the lens of AI and how AI can help humans achieve cooperation. More precisely, \citet{dafoe2020open} classified Cooperative AI research into four broad topics: \emph{Understanding}, \emph{Communication}, \emph{Commitment}, and \emph{Institutions}. They span various disciplines, from game theory to machine learning to social sciences. 
In this survey, we discuss cooperative AI, focusing on reinforcement learning in \S\ref{sec:cooperative-ai-training} and game theory in \S\ref{subsec:formal-ethics-coop}.

\paragraph{Addressing Social Complexities} The requirement of ethicality contains in itself a social component. ``What is ethical'' is often defined within a social context; therefore, its implementation in AI systems also needs to account for social complexities. \citet{critch2020ai} provides proposals for many research topics in this vein. One avenue of research focuses on the realistic simulation of social systems, including rule-based \emph{agent-based modeling} \citep{bonabeau2002agent,de2014agent}, deep learning-based simulation \citep{sert2020segregation,storchan2021learning}, and those incorporating LLMs \citep{park2023generative}. These simulation methods could serve a diverse array of down-stream applications, from impact assessment \citep{calvo2020advancing,fernandes2020adoption,osoba2020steps} to multi-agent social learning \citep{critch2020ai}. On another front, the fields of \emph{social choice} \citep{sen1986social,arrow2012social} and, relatedly, \emph{computational social choice} \citep{brandt2016handbook} have aimed to produce mathematical and computational solutions for preference aggregation in a diverse population, among other goals. It has been argued that a similar approach when combined with human preference-based alignment methods (\textit{e.g.}, RLHF and most other methods introduced in \S\ref{sec:learning-from-feedback}), could supplement these methods to guarantee a fair representation of everyone's preferences \citep{leike2023proposal, CIPwhitepaper}. There have been early-stage experiments on this proposal \citep{yamagata2021reinforcement,bakker2022fine,kopf2023openassistant}. To complement this approach of learning values from crowds, it has also been argued that embodied values in AI systems should undergo continual progress over the long term as opposed to being permanently locked-in \citep{kenward2021machine}, in order to navigate through emerging challenges, as well as to become future-proof and meet potential \emph{unknown unknowns} in the moral realm. 

\subsubsection{AI Safety beyond Alignment}
\label{sec:ai-safety-beyond}
Following the introduction of alignment inner scope, in this section, we further discuss AI safety beyond alignment to enrich our discussion and clarify the alignment scope. AI causes many risks beyond alignment failures. For example, malicious actors could deliberately use AI to cause harm, such as by building biological weapons. Alternatively, competition between AI developers could lead them to neglect risks and race ahead with deploying dangerous AI systems. While this survey paper primarily focuses on alignment, we draw from \citet{hendrycks2023overview} to provide a brief overview of other causes of catastrophic AI risks.

\paragraph{Malicious Use}
Malicious actors can deliberately use AI to cause harm. Already, deepfakes have been used by criminals to enable scams and blackmail \citep{cao2023deepfake}. As AI systems develop more dangerous capabilities, the threat of misuse looms larger. 

Biological weapons provide one concerning example of how AI could be maliciously used to cause harm. Research has shown that large language models can provide detailed, step-by-step instructions about synthesizing pandemic potential pathogens \citep{soice2023large}. In addition to spreading information about how to create biological weapons, AI could help design new pathogens that are more lethal and transmissible than existing illnesses \citep{sandbrink2023artificial}. Terrorist groups such as Aum Shinrikyo \citep{danzig2012aum} have already attempted to build biological weapons in order to cause widespread destruction, and AI could make it easier for small groups to create biological weapons and start global pandemics. 
Other kinds of malicious use could include using AI to launch cyberattacks against critical infrastructure \citep{mirsky2021threat}, or create autonomous agents that survive and spread outside of human control \citep{rogueai}. As new dangerous capabilities arise in AI systems, thorough evaluations will be required to determine how an AI system could be used to cause harm. 

Malicious use should not be considered a failure of alignment because when an AI system behaves according to the intentions of a malicious user, this system would be aligned with its user but would still pose a serious threat to society. Policies to ensure that AI is aligned with the public interest will be essential to avert this threat.

\paragraph{Collective Action Problems}

Many AI developers are racing to build and deploy powerful AI systems \citep{grant2023airace}. This incentivizes developers to neglect safety and race ahead to deploy their AI systems. Even if one developer wants to be careful and cautious, they might fear that slowing down to evaluate their systems and invest in new safety features thoroughly might allow their competition to outpace them \citep{armstrong2013racing}. This creates a social dilemma where individual AI developers and institutions rationally pursuing their own interests can lead to suboptimal outcomes for everyone. Success in competition between AI systems may be governed by evolutionary dynamics, where the strongest and most self-interested AI systems could be the most likely to survive \citep{hendrycks2023natural}. Preventing these collective action problems from causing societal catastrophes could require intervention by national and international AI policies to ensure that all AI developers uphold common safety standards. 



